Webots.HPC: A Parallel Robotics Simulation Pipeline for Autonomous Vehicles on High Performance Computing

In the rapidly evolving and maturing field of robotics, computer simulation has become an invaluable tool in the design process. Webots, a state-of-the-art robotics simulator, is often the software of choice for robotics research. Even so, Webots simulations are often run on personal and lab computers. For projects that would benefit from an aggregated output dataset from thousands of simulation runs, there is no standard recourse; this project sets out to mitigate this by developing a formalized parallel pipeline for running sequences of Webots simulations on powerful HPC resources. Such a pipeline would allow researchers to generate massive datasets from their simulations, opening the door for potential machine learning applications and decision tool development. We have developed a pipeline capable of running Webots simulations both headlessly and in GUI-enabled mode over an SSH X11 server, with simulation execution occurring remotely on HPC compute nodes. Additionally, simulations can be run in sequence, with a batch job being distributed across an arbitrary number of computing nodes and each node having multiple instances running in parallel. The implemented distribution and parallelization are extremely effective, with a 100\% simulation completion rate after 12 hours of runs. Overall, this pipeline is very capable and can be used to extend existing projects or serve as a platform for new robotics simulation endeavors.

==> Makefile <==
#
# makefile
#
# Makefile for LaTeX Documents
#

SHELL=sh

#
# Base name of the document
#
TARGET=thesis

#
# Sources
#
SOURCES=*.tex

# 
# File-extensions to DELETE recursive from here
# 
EXTENSION=aux toc idx ind ilg log out lof lot lol bbl blg



#
# Targets
# 
all: $(TARGET).pdf


#
# Portable Document Format (PDF)
#
$(TARGET).pdf: $(SOURCES)
	@echo "-------------------------------------------------------------------------------"
	@echo "-- Running 'pdflatex $(TARGET).tex'"
	@echo "-------------------------------------------------------------------------------"
	@pdflatex $(TARGET).tex

	@echo ""
	@echo "-------------------------------------------------------------------------------"
	@echo "-- Running 'bibtex $(TARGET)'"
	@echo "-------------------------------------------------------------------------------"
	@bibtex $(TARGET)

	@echo ""
	@echo "-------------------------------------------------------------------------------"
	@echo "-- Rerunning 'pdflatex $(TARGET).tex' to get cross-references right"
	@echo "-------------------------------------------------------------------------------"
	@pdflatex $(TARGET).tex

	@latex_count=5 ; \
	while egrep -s 'Rerun (LaTeX|to get cross-references right)' \
		$(TARGET).log && [ $$latex_count -gt 0 ] ;\
	do \
		echo "";\
		echo "-------------------------------------------------------------------------------";\
		echo "-- Rerunning 'pdflatex $(TARGET).tex' to get cross-references right" ;\
		echo "-------------------------------------------------------------------------------";\
		pdflatex $(TARGET).tex ;\
		latex_count=`expr $$latex_count - 1` ;\
	done

#
# Show in acroread
#
acroread: $(TARGET).pdf
	acroread $(TARGET).pdf&

#
# Show in kpdf
#
kpdf: $(TARGET).pdf
	kpdf $(TARGET).pdf&

#
# Clean
#
clean:
	@for EXT in $(EXTENSION); do \
		find . -name \*\.$${EXT} -exec rm -vf \{\} \; ;\
	done
	@rm -vf $(TARGET).pdf


==> README <==
ClemsonThesis Template README
-----------------------------
This package includes a template for generating a thesis or dissertation
following the style requirements for the Graduate School at Clemson University.

Contents
--------
    1. File Descriptions
    2. Caption Formatting in the 'List of [Figures, Tables, ...]'


1. File Descriptions
--------------------
The files contained in this package serve various purposes.
'ClemsonThesis.cls' is the main document class that defines how things are 
supposed to look.  You should not have to modify this file.

'thesis.tex' is a sample of the main LaTeX document that uses the
'ClemsonThesis' class.  Comments are included in this file to explain what
everything does.  Each section of the document is contained in the following
separate .tex files:

    abstract.tex
    dedication.tex
    acknowledgments.tex
    introduction.tex
    researchDesign.tex
    relatedWork.tex
    results.tex
    conclusions.tex
    appendixA.tex
    appendixB.tex
    appendixC.tex

These files are included by the main 'thesis.tex' file.  Dividing the document
up into separate files that are included by the main file makes it easier to
conditionally build parts of the document (i.e., if you only want to print the
introduction, you can comment out the inclusion of all of the other sections).

'bibliography.bib' is the BibTeX database used by 'thesis.tex'.  That file 
will contain all of the bibliography entries to be cited in the document.  
The one included includes some samples to show you the proper format.  The
file 'introduction.tex' includes examples of how to cite those references
(e.g., \cite{refTag}).

'Makefile' is used to convert the document into a PDF in a UNIX (e.g., MacOS, 
Linux) environment.  If they're using some other environment (e.g., Windows),
whatever tool they choose to use will take care of that for them.

Finally, 'testbed.jpg' is an image that is part of the sample document.  I 
included that as an example of how to include an image in the document.



2. Caption Formatting in the 'List of [Figures, Tables, ...]'
-------------------------------------------------------------
The Graduate School's style guidelines requires that in the 'List of
<Whatever>', when entries are longer than 4.5 inches, that they be split
onto two lines.  Basically, the text should not run all the way to the
page number -- some dots should be included.  The style specification
included in this package does *not* automatically handle this case.  You
*must* review your captions and include appropriate breaks when necessary.

To do this, you can use the '\newline' command.  Here's an example:

    \caption[This is a really really really really really really long caption
             that might need a newline \newline here so I put one in manually]
            {This is a really really really really really really long caption
            that might need a newline here so I put one in manually}

The text between the square brackets (i.e., [ ]) will be shown in the 'List of
<Whatever>', and the text between the curly braces (i.e., { }) will be shown
inline in the text.  The only difference between the two is a '\newline' in
the first that indicates where LaTeX should place the line break.


==> dedication.tex <==
\chapter*{Dedication}



==> relatedWork.tex <==
\chapter{Related and Future Work}
This section will analyze and describe several related works to this paper, and present several avenues for future work. 




==> walkthrough.tex <==
\chapter {Application Walkthrough}

\section{Converting between Docker and Singularity Images}

\section{Running SUMO on Palmetto Cluster}

\section{Running Webots on Palmetto Cluster}

\subsection{Pairing with SUMO Interface}

\section{Uploading Our Usable Image to Your Own Account on the Cluster}

\section{Adding Additional Libraries to Singularity Image}
